Ekar: An Explainable Method for Knowledge Aware Recommendation

This paper studies recommender systems with knowledge graphs, which can effectively address the problems of data sparsity and cold start. Recently, a variety of methods have been developed for this problem, which generally try to learn effective representations of users and items and then match items to users according to their representations. Though these methods have been shown quite effective, they lack good explanations, which are critical to recommender systems. In this paper, we take a different route and propose generating recommendations by finding meaningful paths from users to items. Specifically, we formulate the problem as a sequential decision process, where the target user is defined as the initial state, and the edges on the graphs are defined as actions. We shape the rewards according to existing state-of-the-art methods and then train a policy function with policy gradient methods. Experimental results on three real-world datasets show that our proposed method not only provides effective recommendations but also offers good explanations.

==> 4-model-old.tex <==
\section{methodology}

\begin{figure*}
\centering
\includegraphics[width=0.96\linewidth]{figures/model_v4.pdf}
\vspace{-10pt}
\caption{A schematic view of our proposed \name\ model. We formulate the generation of explainable paths as a sequential decision process. The user-item-entity graph is the RL environment and a policy network interacts with it. To stabilize training and encourage the agent to explore diverse paths, we design a well-shaped reward.}\label{fig::model}
\end{figure*}



In this section, we describe our proposed \name\ model for path-based explainable recommendation task in detail.

Overall, we formulate the generation of explainable paths as a Markov Decision Process (MDP) on the user-item-entity graph, and we use deep reinforcement learning to solve it. As shown in Figure~\ref{fig::model}, the user-item-entity is treated as the environment, from which we get the observation $s_t$, i.e., a sequence of visited nodes and edges. Based on the encoded state $\mathbf{s}_t$, a policy network consisting of two fully-connected layers outputs the probability distribution over possible action space. Finally, we define the reward being $+1$ if our agent successfully finds those items consumed by the target users $u$ in history. Furthermore, we augment the rewards based on pre-trained state-of-the-art KGE models for the purpose of stabilizing training and encouraging the agent to explore diverse recommendation paths.


%Overall, we first formulate the generation of explainable paths as a Markov Decision Process (MDP) (i.e., Section~\ref{subsec::mdp}). Specifically, the state in our recommendation MDP is defined as the visited nodes and edges sequence. We further define the action space as the set of outgoing edges of last node in state sequence. Given the previous state and the taken action, we use a deterministic transition function to get the new state of MDP. Since our ultimate goal is to find relevant items for recommendation, we define the reward being positive if the terminal nodes are those items consumed by users in history. Afterwards, we solve the aforementioned MDP using policy gradient method (i.e., Section~\ref{subsec::drl}), which learns a policy to master the walks on graph $\mathcal{G}'$.

%\textcolor{red}{We propose to generate meaningful paths from the target user to relevant items, which are able to provide effective recommendations and good explanations at the same time. We formulate the problem as a sequential decision process and train an agent to walk on the graph with policy gradient methods.} 
%The key idea behind \name\ is to generate meaningful paths from users to relevant items, where the generation of such paths are formulated as a Markov Decision Process (MDP). We further solve this MDP using deep reinforcement learning. 

%We formally denote users and items with $\mathcal{U}=\{u_1, u_2, ..., u_N\}$ and $\mathcal{I}=\{i_1, i_2, ..., i_M\}$ respectively. The interactions between users and items are represented as a bipartite graph $\mathcal{G}={\mathcal{U},\mathcal{I},\mathcal{E}}$,   

\subsection{Formulating recommendation as a Markov Decision Process}\label{subsec::mdp}
There are some existing methods~\cite{Wang2018ExplainableRO} trying to find meaningful paths between users and items. These methods first sample a collection of paths with breadth-first or depth-first search strategy and then measure the meaningfulness of the paths with a classification or ranking model. However, the number of possible paths between a user and an item could be exponentially large, and sampling a few of them could miss the meaningful ones. 
Moreover, the paths sampled through BFS or DFS strategy may not always be meaningful. 
%Besides, paths obtained by BFS or DFS may not be always meaningful. 
In this paper, we take a different route and formulate the problem as a sequential decision making problem on the user-item-entity graph $\mathcal{G}'$. We aim to train an agent to walk on $\mathcal{G}'$ to find relevant items.
%\textcolor{red}{Zhu: I revised some. Please check this paragraph.}
%Since the generation of path follows a Markov process, we formulate the problem as a sequential decision making process on the user-item-entity graph $\mathcal{G}'$. Particularly, we train an agent to perform a walk on $\mathcal{G}'$.
Starting from a target user $u$, the agent sequentially selects the next neighbor on the integrated user-item-entity graph $\mathcal{G}'$ until it reaches the predefined maximum number of steps $T$.
%In this way, the agent can efficiently learn to perform long walks, without traversing all possible paths.
Formally, we define the states, actions, transition, and rewards of the Markov Decision Process as follows:

\vspace{3pt}
\xhdr{States} We represent the state as the sequence of traversed relations and entities so far, i.e., $s_t=(r_0, e_0, r_1, e_1, ..., r_t, e_t)\in \mathcal{S}_t$, where $r_t\in \mathcal{R}'$ and $e_t\in \mathcal{V}'$ are relations and entities respectively. 
The initial state $s_0=(r_0, e_0)$ represents the target user, and $r_0$ is an artificially introduced relation to be consistent with other $(r_t, e_t)$ pairs.
%The initial state $s_0=(r_0, e_0)$, where $r_0$ is an artificially introduced relation and $e_0\in \mathcal{U}$ is a user, represents the user to whom we are recommending items.

\vspace{3pt}
\xhdr{Actions} When the agent is under state $s_t$, it can choose an outgoing edge of entity $e_t$ as its next action.
Formally, we define the possible actions under state $s_t$ as $\mathcal{A}_t=\{a=(r', e')|(e_t, r', e')\in \mathcal{G}'\}$.

\vspace{3pt}
\xhdr{Transition} For the state transition $\mathcal{P}(\mathcal{S}_{t+1}=s|\mathcal{S}_t=s_t, \mathcal{A}_t=a_t)$, we adopt a deterministic strategy and simply extend the current state $s_t$ by adding the new action $a_t=(r_{t+1}, e_{t+1})$ as the next state, i.e., $s_{t+1}=(r_0, e_0, ..., r_t, e_t, r_{t+1}, e_{t+1})$.
%We adopt a deterministic state transition for $\mathcal{P}(\mathcal{S}_{t+1}=s|\mathcal{S}_t=s_t, \mathcal{A}_t=a_t)$, where we simply extend state $s_t$ with taken action $a_t=(r_{t+1}, e_{t+1})$. Concretely, the new state is $s_{t+1}=(r_0, e_0, ..., r_t, e_t, r_{t+1}, e_{t+1})$.

\vspace{3pt}
\xhdr{Rewards} No intermediate reward is provided for $(s_{t<T}, a_{t<T})$. The final reward depends on whether or not the agent correctly finds interacted items of the user $u$.
Given the terminal entity $e_T$, the final reward $R_T$ is $+1$ if user $e_0$ has interacted with $e_T$, $0$ if $e_T$ is an item but user $e_0$ has not interacted with it and $-1$ if $e_T$ is not an item-type entity.
%1) $+1$, if $<e_0, ``Interact'' e_T>$ exists in $\mathcal{G}'$; 2) 0, if  otherwise $-1$. 
%\textcolor{red}{(Should we mention that it is just the basic reward function? --dzj) }

\subsection{Solving recommendation MDP with policy-based reinforcement learning}\label{subsec::drl}
Next, we introduce a deep policy-based reinforcement learning method to solve the above MDP. The learned policy is then used to generate recommendations and explanations during inference.
%We further parameterize the above MDP with deep neural networks and optimize it with policy gradient methods.

\subsubsection{The architecture of policy network} Since there are usually millions of entities and hundreds of relations in user-item-entity graph $\mathcal{G}'$, it is almost impossible to utilize discrete states and actions directly, the number of which is exponential to the number of symbolic atoms in $s_t$ and $a_t$ respectively. We, therefore, choose to represent entities and relations in $\mathcal{G}'$ with low-dimensional embeddings. Each action $a=(r, e)$ is represented as the concatenation of relation and entity embeddings, i.e., $\mathbf{a}=[\mathbf{r}';\mathbf{e}']$. The state $s_t=(r_0, e_0, ..., r_t, e_t)$ is encoded by an LSTM~\cite{hochreiter1997long}:% as follows:
\begin{equation}
\begin{aligned}   
    \mathbf{s}_{0} &= \textit{LSTM}(\mathbf{0}, [\mathbf{r}_0; \mathbf{e}_0]), \\
    \mathbf{s}_t &= \textit{LSTM}(\mathbf{s}_{t-1}, [\mathbf{r}_{t}; \mathbf{e}_t]), t>0\\
    %\mathbf{s}_t &= [\mathbf{e_t};\mathbf{h_t}],
\end{aligned}
\end{equation}
%\vspace{-5pt}
where $\mathbf{0}$ is a zero vector and $\mathbf{s}_t$ is the low-dimensional representation of state $s_t$. 
%Besides dimension reduction, another advantage of using continuous representations of state and action lies in valuable semantic information captured by the compact embeddings and LSTM encoder. 







According to our initial definition of rewards, the agent gets a positive reward if and only if it successfully finds the target item. However, this might be problematic for a few reasons: First, for a large user-item-entity graph $\mathcal{G}'$, it is very difficult for the agent to reach the correct items due to the huge search space, especially at the beginning of training~\cite{xiong2017deeppath}. In other words, the rewards will be very sparse. As a result, the learning process of the agent could be very inefficient and take a long time to converge. Second, the goal of recommender systems is to infer new items that users are likely to interact with in the future, rather than repeating users' historical items. However, receiving positive rewards only from historical items discourages the agent to explore new paths and items, which should be the target of recommender systems. To accelerate the training process and meanwhile encourage the agent to explore items that have not been purchased or rated by the target user, 
%we first learn representations of $\mathcal{V}'$ and $\mathcal{R}'$ by applying knowledge graph embedding methods (e.g., TransE~\cite{bordes2013translating} or ConvE~\cite{dettmers2018convolutional}) on $\mathcal{G}'$ and propose to shape the rewards~\cite{ng1999policy} in the following way:
we propose to shape the rewards~\cite{ng1999policy} in the following way: 
\begin{equation}
    R_T = 
    \begin{cases}
    1, & \text{if } e_T\in \mathcal{I} \text{ and } <e_0, \bar{r}, e_T> \in \mathcal{G}', \\
    \sigma(\psi(e_0, \bar{r}, e_T)),
    %f(\mathbf{e_0}, \mathbf{e}_T),
    & \text{if } e_T\in \mathcal{I} \text{ and } <e_0, \bar{r}, e_T> \notin \mathcal{G}', \\
    -1 , & \text{otherwise},
    \end{cases}
    \label{eq:reward}
\end{equation}
%\vspace{-1pt}
where $\sigma(x)=\frac{1}{1+e^{(-x)}}$ is the sigmoid function and $\bar{r}$ represents the relation ``Interact''.
$\psi(e_0, \bar{r}, e_T)$ is the score function that measures the correlation between user $e_0$ and the searched item $e_T$. In our study, $\psi(e_0, \bar{r}, e_T)$ is pre-trained by maximizing the likelihood of all triplets in graph $\mathcal{G}'$ and can be the score function of any state-of-the-art knowledge graph embedding models~\cite{dettmers2018convolutional,yang2014embedding,sun2019rotate}. For example, the score function is $\psi(e_0, \bar{r}, e_T)=-\|e_0 + \bar{r} - e_T \|$ in TransE~\cite{bordes2013translating} model.
Different from the original rewards defined in Section~\ref{subsec::mdp}, items that the target user has not interacted with now receive positive rewards, which are determined by the pre-trained knowledge graph embeddings.
%wherein the score function $\psi(e_0, e_T)$ is learned by maximizing the likelihood of triplets in user-item-entity graph $\mathcal{G}'$.
%where $\sigma(x)=\frac{1}{1+e^{(-x)}}$ is the sigmoid function and $\psi(e_0, e_T)$ is the score function of used knowledge graph embedding method. For example, the score function of TransE is $\psi(e_0, e_T)=-\Vert \mathbf{e_0} + \mathbf{r} - \mathbf{e_T} \Vert$, where $\mathbf{e_0}$, $\mathbf{e_T}$ and $\mathbf{r}$ are representations of entity $e_0$, entity $e_T$ and relation ``Interact''.
%where $\mathbf{e_0}$ and $\mathbf{e}_T$ are embeddings of user $e_0$ and entity $e_T$ learned by knowledge graph embedding methods (e.g., ConvE~\cite{dettmers2018convolutional} or DistMult~\cite{yang2014embedding}) respectively, and $f(\cdot, \cdot) \in (0, 1)$ is a score function to measure the correlation between $e_0$ and $e_T$. For simplicity, we use a sigmoid function here: $f(\mathbf{e}_0, \mathbf{e}_T)=\frac{1}{1+e^{(-\mathbf{e}_0^\top \mathbf{e}_T))}}$.


\subsubsection{Policy Network}
%\textcolor{blue}{Q-learning~\cite{watkins1992q} and policy gradient~\cite{sutton2000policy} are two popular methods for deep reinforcement learning problems.} 
In this paper, we use the policy gradient method to solve the proposed recommendation MDP.
%\textcolor{blue}{because Q-learning may need lots of samples to converge due to the huge state space in our task.}
Based on parameterized state $\mathbf{s}_t$ and parameterized action $\mathbf{a}$, we calculate the probability distribution over possible action $\mathcal{A}_t$ as follows:
\begin{equation}
    \begin{aligned}
    & \mathbf{y}_t = \mathbf{W}_2 \textit{ReLU}(\mathbf{W}_1\mathbf{s}_t + \mathbf{b}_1) + \mathbf{b}_2, \\
    & \pi_\theta(a'|s_t) = \frac{\exp({\mathbf{a}'}^\top \mathbf{y}_t)}{\sum_{a\in \mathcal{A}_t}\exp(\mathbf{a}^\top \mathbf{y}_t)},
    \end{aligned}
\end{equation}
where \{$\mathbf{W}_1, \mathbf{W}_2$\} and \{$\mathbf{b}_1, \mathbf{b}_2$\} are weight matrices and weight vectors of a two-layer fully-connected neural network, $\textit{ReLU}(x)=\textit{max}(0, x)$ is the non-linear activation function and $\pi_\theta(a'|s_t)$ is the probability of taken action $a'$ under state $s_t$.

\subsubsection{Optimization} During training, the agent starts with an initial state $(r_0, e_0)$, where $e_0$ is the target user, and sequentially extends its path to a maximum length of $T$. We then use the reward function (i.e., Eq.~\ref{eq:reward}) to assign the trajectory $(s_0, a_0, s_1, a_1, ..., s_T)$ a final reward. Formally, we define the expected rewards over all traversed paths of all users as:
\begin{equation}
    J(\theta)= \E_{e_0\in \mathcal{U}}[\E_{a_1, a_2, ..., a_T\sim \pi_\theta(a_t|s_t)}[R_T]].
\end{equation}
which is maximized via gradient ascent, and the gradients of all parameters $\theta$ are derived by the REINFORCE~\cite{williams1992simple} algorithm, i.e.,
\begin{equation}
    \bigtriangledown_{\theta} J(\theta) \approx \bigtriangledown_{\theta} \sum_{t} R_T\log \pi_\theta(a_t|s_t).
\end{equation}


